S2CTrans: Building a bridge from SPARQL to Cypher

In graph data applications, data is primarily maintained using two models: RDF (Resource Description Framework) and property graph. The property graph model is widely adopted by industry, leading to property graph databases generally outperforming RDF databases in graph traversal query performance. However, users often prefer SPARQL as their query language, as it is the W3C's recommended standard. Consequently, exploring SPARQL-to-Property-Graph-Query-Language translation is crucial for enhancing graph query language interoperability and enabling effective querying of property graphs using SPARQL. Despite the substantial differences in semantic representation and processing logic between SPARQL and property graph query languages like Cypher, this paper demonstrates the feasibility of translating SPARQL to Cypher for graph traversal queries using graph relational algebra. We present the S2CTrans framework, which achieves SPARQL-to-Cypher translation while preserving the original semantics. Experimental results with the Berlin SPARQL Benchmark (BSBM) datasets show that S2CTrans successfully converts most SELECT queries in the SPARQL 1.1 specification into type-safe Cypher statements, maintaining result consistency and improving the efficiency of data querying using SPARQL.

==> related-work-at-last.tex <==
\section{Related Work}
	W3C Workshop on Web Standardization for Graph Data in 2019 calls for building a bridge between RDF and property graph. Participants agreed on the importance of developing standard methods to allow interoperability between RDF and property graph database systems. Aiming at the interoperability of knowledge graph\cite{InteroperabilityBook}\cite{interoperability}, we briefly summarize the related work of knowledge graph query language translation: 
	
	\textbf{SPARQL-to-SQL. }
	Artem Chebotko et al. \cite{SematicPreserving} proposed the first provably semantics preserving SPARQL-to-SQL translation. They formalized a relational algebra based semantics of SPARQL and proved that it is equivalent to the mapping-based semantics of SPARQL. Their translation method is generic and can be directly applied to existing RDBMS-based RDF stores.
	
	\textbf{SQL-to-SPARQL. }
	Jyothsna Rachapalli et al. \cite{RETRO} proposed a semantic-preserving SQL-to-SPARQL transformation framework RETRO, and based on the combined semantics of the two query languages, gave a proof of the correctness of this transformation. Mohamed Bahaj et al. \cite{LeftOuter} established an effective semantic transformation algorithm for the shortcomings of the transformation from SQL to SPARQL left outer join operation, and integrated it in RETRO.
	
	\textbf{Cypher-to-SQL. }
	Marton Elekes et al. \cite{operCypher2SQL} intended to use expressive graph query language and take advantage of the performance of existing relational databases to develop a transpiler for transforming openCypher graph queries into SQL statements, which was evaluated and analyzed in detail.
	
	\textbf{SPARQL-to-Gremlin. }
	Thakkar et al. \cite{2020Let}\cite{2018Two} designed a translator for SPARQL 2 Gremlin. Jena ARQ \cite{2006Jena} parses SPARQL to generate AST, and then maps it to Gremlin traversal according to the graph pattern and modifier in AST. However, it only supports SPARQL 1.0, and the query types provided are not comprehensive.
	
	\textbf{SPARQL-to-Cypher. }
	Moreira et al. \cite{SPARQLing} describe a mapping method from SPARQL to Cypher, but the mapping still has some syntax and keywords that have not yet been implemented, and the obtained Cypher statements become very redundant.
 
